Parallel Key-Value Cache Fusion for Position Invariant RAG

Recent advancements in Large Language Models (LLMs) underscore the necessity of Retrieval Augmented Generation (RAG) to leverage external information. However, LLMs are sensitive to the position of relevant information within contexts and tend to generate incorrect responses when such information is placed in the middle, known as `Lost in the Middle' phenomenon. In this paper, we introduce a framework that generates consistent outputs for decoder-only models, irrespective of the input context order. Experimental results for three open domain question answering tasks demonstrate position invariance, where the model is not sensitive to input context order, and superior robustness to irrelevent passages compared to prevailing approaches for RAG pipelines.

==> tables/appen-ins.tex <==


% \begin{table*}[!t]
%     \renewcommand{\arraystretch}{1.15}
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{p{3.1cm} XXXXX XXXXX XXXXX}
%         \toprule
%         \textbf{Dataset}    & \multicolumn{4}{c}{\textbf{NQ}}   & \multicolumn{4}{c}{\textbf{TQA}}  & \multicolumn{4}{c}{\textbf{POPQA}}  \\
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
%         \textbf{Top-K} & 5 & 10 & 20 & 40 & 5 & 10 & 20 & 40 & 5 & 10 & 20 & 40    \\
%         \midrule
%         % \multicolumn{14}{l}{\llama-2-7B} \\
%         \llama  &\scriptsize{34.1}  &\scriptsize{37.2} &\scriptsize{40.4} &\scriptsize{38.8}  &\scriptsize{62.4} &\scriptsize{66.5} &\scriptsize{67.2} &\scriptsize{64.7}  
%         &\scriptsize{31.7} &\scriptsize{33.7} &\scriptsize{33.7} &\scriptsize{31.6}\\
%         \llamaone  &\scriptsize{43.2}  &\scriptsize{41.5} &\scriptsize{42.7} &\scriptsize{42.4}   &\scriptsize{64.0} &\scriptsize{64.8} &\scriptsize{65.9} &\scriptsize{67.1} 
%         &\scriptsize{31.1} &\scriptsize{33.4} &\scriptsize{32.8} &\scriptsize{33.3}\\
        
%         \llamains  &\scriptsize{48.5}  &\scriptsize{51.5} &\scriptsize{50.3} &\scriptsize{43.9}  &\scriptsize{61.1} &\scriptsize{61.0} &\scriptsize{62.3} &\scriptsize{56.1}  
%         &\scriptsize{24.4} &\scriptsize{24.3} &\scriptsize{25.2} &\scriptsize{22.0}\\
%         \llamaoneins  &\scriptsize{48.2}  &\textbf{\scriptsize{52.3}} &\textbf{\scriptsize{54.0}} &\textbf{\scriptsize{54.8}}   &\scriptsize{66.8} &\textbf{\scriptsize{70.3}} &\textbf{\scriptsize{71.2}} &\textbf{\scriptsize{72.5}} &\scriptsize{30.2} &\scriptsize{34.3} &\scriptsize{36.9} &\scriptsize{38.2}\\
        
%         \hdashline
%         \kvllamaT  &\scriptsize{51.6}  &\scriptsize{51.7} &\scriptsize{51.4} &\scriptsize{49.8} &\scriptsize{67.5}  &\scriptsize{68.8} &\scriptsize{69.3} &\scriptsize{69.3} &\scriptsize{44.5} &\scriptsize{46.7} &\textbf{\scriptsize{48.3}} &\textbf{\scriptsize{46.7}} \\
%         \kvllamaoneT  &\textbf{\scriptsize{51.7}}  &\scriptsize{51.8} &\scriptsize{50.8} &\scriptsize{49.0}  &\textbf{\scriptsize{68.6}}  &\scriptsize{68.3} &\scriptsize{69.3} &\scriptsize{68.7} &\textbf{\scriptsize{44.7}} &\textbf{\scriptsize{47.6}} &\scriptsize{47.4} &\scriptsize{45.3} \\
%         % \kvllamaTall  &\scriptsize{-}  &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-}  &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} \\
%         % \kvllamaoneTall  &\scriptsize{-}  &\scriptsize{-} &\scriptsize{-} &\scriptsize{-}  &\scriptsize{-}  &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Accuracy comparison with differnet position-invariant readers. Across top-k results, KV-fusion maintains stable and the strong accuracies, while other models either degrade or exhibit relatively low accuracies.}
%     \label{tab:exp-ins}
% \end{table*}

% \begin{table*}[!t]
%     \renewcommand{\arraystretch}{1.15}
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{p{3.1cm} XXXXX XXXXX XXXXX}
%         \toprule
%         \textbf{Dataset}    & \multicolumn{5}{c}{\textbf{NQ}}   & \multicolumn{5}{c}{\textbf{TQA}}  & \multicolumn{5}{c}{\textbf{POPQA}}  \\
%         \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} 
%         \textbf{Top-K} & 1 & 5 & 10 & 20 & 40 & 1 & 5 & 10 & 20 & 40  & 1 & 5 & 10 & 20 & 40    \\
%         \midrule
%         % \multicolumn{14}{l}{\llama-2-7B} \\
%         \llama  &\scriptsize{40.0}  &\scriptsize{34.1}  &\scriptsize{37.2} &\scriptsize{40.4} &\scriptsize{38.8}  &\scriptsize{61.4}  &\scriptsize{62.4} &\scriptsize{66.5} &\scriptsize{67.2} &\scriptsize{64.7}  &\scriptsize{29.5}  &\scriptsize{31.7} &\scriptsize{33.7} &\scriptsize{33.7} &\scriptsize{31.6}\\
%         \llamaone  &\scriptsize{43.1}  &\scriptsize{43.2}  &\scriptsize{41.5} &\scriptsize{42.7} &\scriptsize{42.4}  &\scriptsize{62.1}  &\scriptsize{64.0} &\scriptsize{64.8} &\scriptsize{65.9} &\scriptsize{67.1} &\scriptsize{30.7}  &\scriptsize{31.1} &\scriptsize{33.4} &\scriptsize{32.8} &\scriptsize{33.3}\\
%         % \llama  &\scriptsize{40.0}  &\scriptsize{34.1}  &\scriptsize{37.2} &\scriptsize{40.4} &\scriptsize{38.8}  &\scriptsize{61.4}  &\scriptsize{62.4} &\scriptsize{66.5} &\scriptsize{67.2} &\scriptsize{64.7}  &\scriptsize{-}  &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-}\\
%         % \llama  &\scriptsize{40.0}  &\scriptsize{34.1}  &\scriptsize{37.2} &\scriptsize{40.4} &\scriptsize{38.8}  &\scriptsize{61.4}  &\scriptsize{62.4} &\scriptsize{66.5} &\scriptsize{67.2} &\scriptsize{64.7}  &\scriptsize{-}  &\scriptsize{-} &\scriptsize{-} &\scriptsize{-} &\scriptsize{-}\\
%         \hdashline
%         \replug &\scriptsize{36.8}  &\scriptsize{35.6}  &\scriptsize{34.0} &\scriptsize{33.6} &\scriptsize{32.2}  &\scriptsize{57.8}  &\scriptsize{57.7}  &\scriptsize{56.4} &\scriptsize{55.8} &\scriptsize{56.3} &\scriptsize{30.0}  &\scriptsize{30.1}  &\scriptsize{28.1} &\scriptsize{26.0} &\scriptsize{26.7} \\
%         \replugone &\scriptsize{40.1}  &\scriptsize{38.6}  &\scriptsize{36.4} &\scriptsize{35.3} &\scriptsize{34.1}  &\scriptsize{63.7} &\scriptsize{65.1}  &\scriptsize{64.4} &\scriptsize{62.8} &\scriptsize{60.6} &\scriptsize{33.0}  &\scriptsize{35.4}  &\scriptsize{33.8} &\scriptsize{30.7} &\scriptsize{29.4} \\
%         \PAMQA  &\scriptsize{44.1} &\textbf{\scriptsize{51.9}}  &\scriptsize{46.5} &\scriptsize{40.7} &\scriptsize{19.7}  &\scriptsize{61.3}  &\scriptsize{65.9}  &\scriptsize{61.2} &\scriptsize{52.3} &\scriptsize{29.0} &\scriptsize{30.0}  &\scriptsize{37.0} &\scriptsize{35.9} &\scriptsize{34.9} &\scriptsize{15.7} \\
%         \kvllamaT  &\scriptsize{44.4} &\scriptsize{51.6}  &\scriptsize{51.7} &\textbf{\scriptsize{51.4}} &\textbf{\scriptsize{49.8}}  &\scriptsize{59.3}  &\textbf{\scriptsize{69.2}}  &\textbf{\scriptsize{68.9}} &\textbf{\scriptsize{69.7}} &\scriptsize{68.5} &\scriptsize{34.0}  &\scriptsize{44.5} &\scriptsize{46.7} &\textbf{\scriptsize{48.3}} &\textbf{\scriptsize{46.7}} \\
%         \kvllamaoneT  &\textbf{\scriptsize{45.9}} &\scriptsize{51.7}  &\textbf{\scriptsize{51.8}} &\scriptsize{50.8} &\scriptsize{49.0}  &\textbf{\scriptsize{63.7}}  &\scriptsize{68.6}  &\scriptsize{68.3} &\scriptsize{69.3} &\textbf{\scriptsize{68.7}} &\textbf{\scriptsize{35.3}}  &\textbf{\scriptsize{44.7}} &\textbf{\scriptsize{47.6}} &\scriptsize{47.4} &\scriptsize{45.3} \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Accuracy comparison with other position-invariant methods. Across top-k results, KV-fusion maintains stable and the strong accuracies, while other models either degrade or exhibit relatively low accuracies.}
%     \vspace{-5mm}
%     \label{tab:exp2}
% \end{table*}


% before haystack
% \begin{table*}[!t]
%     \renewcommand{\arraystretch}{1.15}
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{p{2.9cm} XXXXX XXXXX XXXXX}
%         \toprule
%         \textbf{Dataset}    & \multicolumn{5}{c}{\textbf{NQ}}   & \multicolumn{5}{c}{\textbf{TQA}}  & \multicolumn{5}{c}{\textbf{POPQA}}  \\
%         \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} 
%         \textbf{Top-K} & 1 & 5 & 10 & 20 & 40 & 1 & 5 & 10 & 20 & 40  & 1 & 5 & 10 & 20 & 40    \\
%         \midrule
%         % \multicolumn{14}{l}{\llama-2-7B} \\
%         \llama  &\scriptsize{43.5}  &\scriptsize{46.0}  &\scriptsize{47.1} &\scriptsize{46.9} &\scriptsize{46.0}  &\scriptsize{65.7}  &\scriptsize{69.1} &\scriptsize{70.3} &\scriptsize{69.7}&\scriptsize{66.1}  &\scriptsize{33.6}  &\scriptsize{40.2} &\scriptsize{40.2} &\scriptsize{41.0} &\scriptsize{41.9}\\
%         \llamaone  &\scriptsize{45.1}  &\scriptsize{48.8}  &\scriptsize{48.9} &\scriptsize{48.8} &\scriptsize{47.6}  &\textbf{\scriptsize{66.1}}  &\textbf{\scriptsize{69.4}} &\textbf{\scriptsize{70.4}} &\textbf{\scriptsize{70.9}}&\textbf{\scriptsize{72.1}} &\scriptsize{33.2}  &\scriptsize{39.8} &\scriptsize{41.2} &\scriptsize{42.4} &\scriptsize{42.2}\\
%         \hdashline
%         \replug &\scriptsize{36.8}  &\scriptsize{35.6}  &\scriptsize{34.0} &\scriptsize{33.6} &\scriptsize{32.2}  &\scriptsize{57.8}  &\scriptsize{57.7}  &\scriptsize{56.4} &\scriptsize{55.8} &\scriptsize{56.3} &\scriptsize{30.0}  &\scriptsize{30.1}  &\scriptsize{28.1} &\scriptsize{26.0} &\scriptsize{26.7} \\
%         \replugone &\scriptsize{40.1}  &\scriptsize{38.6}  &\scriptsize{36.4} &\scriptsize{35.3} &\scriptsize{34.1}  &\scriptsize{63.7}  &\scriptsize{65.1}  &\scriptsize{64.4} &\scriptsize{62.8} &\scriptsize{60.6} &\scriptsize{33.0}  &\scriptsize{35.4}  &\scriptsize{33.8} &\scriptsize{30.7} &\scriptsize{29.4} \\
%         \PAMQA  &\scriptsize{44.1} &\textbf{\scriptsize{51.9}}  &\scriptsize{46.5} &\scriptsize{40.7} &\scriptsize{19.7}  &\scriptsize{61.3}  &\scriptsize{65.9}  &\scriptsize{61.2} &\scriptsize{52.3} &\scriptsize{29.0} &\scriptsize{30.0}  &\scriptsize{37.0} &\scriptsize{35.9} &\scriptsize{34.9} &\scriptsize{15.7} \\
%         \kvllamaT  &\scriptsize{44.4} &\scriptsize{51.6}  &\scriptsize{51.7} &\textbf{\scriptsize{51.4}} &\textbf{\scriptsize{49.8}}  &\scriptsize{59.3}  &\scriptsize{69.2}  &\scriptsize{68.9} &\scriptsize{69.7} &\scriptsize{68.5} &\scriptsize{34.0}  &\scriptsize{44.5} &\scriptsize{46.7} &\textbf{\scriptsize{48.3}} &\textbf{\scriptsize{46.7}} \\
%         \kvllamaoneT  &\textbf{\scriptsize{45.9}} &\scriptsize{51.7}  &\textbf{\scriptsize{51.8}} &\scriptsize{50.8} &\scriptsize{49.0}  &\scriptsize{63.7}  &\scriptsize{68.6}  &\scriptsize{68.3} &\scriptsize{69.3} &\scriptsize{68.7} &\textbf{\scriptsize{35.3}}  &\textbf{\scriptsize{44.7}} &\textbf{\scriptsize{47.6}} &\scriptsize{47.4} &\scriptsize{45.3} \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Accuracy comparison with other position-invariant methods. As top-k increases, baseline models experience a sharp decline in accuracy. In contrast, KV-fusion exhibits a more gradual decrease in accuracy, ranging from 2\% to 5\% between top-20 and top-40 contexts.}
%     \vspace{-5mm}
%     \label{tab:exp2}
% \end{table*}


% % \begin{table*}[!t]
% %     \renewcommand{\arraystretch}{1.15}
% %     \centering
% %     \small
% %     \begin{tabularx}{\textwidth}{p{2.9cm} XXXXX XXXXX XXXXX}
% %         \toprule
% %         \textbf{Dataset}    & \multicolumn{5}{c}{\textbf{NQ}}   & \multicolumn{5}{c}{\textbf{TQA}}  & \multicolumn{5}{c}{\textbf{POPQA}}  \\
% %         \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} 
% %         \textbf{Top-K} & 1 & 5 & 10 & 20 & 40 & 1 & 5 & 10 & 20 & 40  & 1 & 5 & 10 & 20 & 40    \\
% %         \midrule
% %         % \multicolumn{14}{l}{\llama-2-7B} \\
% %         \llama  &\scriptsize{43.5}  &\scriptsize{46.0}  &\scriptsize{47.1} &\scriptsize{46.9} &\scriptsize{46.0}  &\scriptsize{65.7}  &\scriptsize{69.1} &\scriptsize{70.3} &\scriptsize{69.7}&\scriptsize{66.1}  &\scriptsize{33.6}  &\scriptsize{40.2} &\scriptsize{40.2} &\scriptsize{41.0} &\scriptsize{41.9}\\
% %         \llamaone  &\scriptsize{45.1}  &\scriptsize{48.8}  &\scriptsize{48.9} &\scriptsize{48.8} &\scriptsize{47.6}  &\textbf{\scriptsize{66.1}}  &\textbf{\scriptsize{69.4}} &\textbf{\scriptsize{70.4}} &\textbf{\scriptsize{70.9}}&\textbf{\scriptsize{72.1}} &\scriptsize{33.2}  &\scriptsize{39.8} &\scriptsize{41.2} &\scriptsize{42.4} &\scriptsize{42.2}\\
% %         \hdashline
% %         \replug &\scriptsize{12.8}  &\scriptsize{16.9}  &- &- &-  &\scriptsize{23.4}  &\scriptsize{28.7}  &- &- &- &\scriptsize{9.0}  &\scriptsize{13.5}  &- &- &- \\
% %         \replugone &\scriptsize{12.6}  &\scriptsize{17.0}  &\scriptsize{18.9} &- &-  &\scriptsize{23.7}  &\scriptsize{29.1}  &\scriptsize{31.3} &- &- &\scriptsize{8.7}  &\scriptsize{13.8}  &\scriptsize{15.0} &- &- \\
% %         \PAMQA  &\scriptsize{44.1} &\textbf{\scriptsize{51.9}}  &\scriptsize{46.5} &\scriptsize{40.7} &\scriptsize{19.7}  &\scriptsize{61.3}  &\scriptsize{65.9}  &\scriptsize{61.2} &\scriptsize{52.3} &\scriptsize{29.0} &\scriptsize{30.0}  &\scriptsize{37.0} &\scriptsize{35.9} &\scriptsize{34.9} &\scriptsize{15.7} \\
% %         \rowcolor{gray!25}
% %         \kvllamaT  &\scriptsize{44.4} &\scriptsize{51.6}  &\scriptsize{51.7} &\textbf{\scriptsize{51.4}} &\textbf{\scriptsize{49.8}}  &\scriptsize{59.3}  &\scriptsize{69.2}  &\scriptsize{68.9} &\scriptsize{69.7} &\scriptsize{68.5} &\scriptsize{34.0}  &\scriptsize{44.5} &\scriptsize{46.7} &\textbf{\scriptsize{48.3}} &\textbf{\scriptsize{46.7}} \\
% %         \kvllamaoneT  &\textbf{\scriptsize{45.9}} &\scriptsize{51.7}  &\textbf{\scriptsize{51.8}} &\scriptsize{50.8} &\scriptsize{49.0}  &\scriptsize{63.7}  &\scriptsize{68.6}  &\scriptsize{68.3} &\scriptsize{69.3} &\scriptsize{68.7} &\textbf{\scriptsize{35.3}}  &\textbf{\scriptsize{44.7}} &\textbf{\scriptsize{47.6}} &\scriptsize{47.4} &\scriptsize{45.3} \\
% %         \bottomrule
% %     \end{tabularx}
% %     \caption{Accuracy comparison with other position-invariant methods in the RAG pipeline. As top-k increases, baseline models experience a sharp decline in accuracy. In contrast, KV-fusion exhibits a more gradual decrease in accuracy, ranging from 2\% to 5\% between top-20 and top-40 contexts.}
% %     \vspace{-5mm}
% %     \label{tab:exp2}
% % \end{table*}

% % \begin{table*}[!t]
% %     \renewcommand{\arraystretch}{1.15}
% %     \centering
% %     \small
% %     \begin{tabularx}{\textwidth}{p{2.9cm} *{5}{>{\centering\arraybackslash}X} *{5}{>{\centering\arraybackslash}X} *{5}{>{\centering\arraybackslash}X}}
% %         \toprule
% %         \textbf{Dataset}    & \multicolumn{5}{c}{\textbf{NQ}}   & \multicolumn{5}{c}{\textbf{TQA}}  & \multicolumn{5}{c}{\textbf{POPQA}}  \\
% %         \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} 
% %         \textbf{Top-K} & 1 & 5 & 10 & 20 & 40 & 1 & 5 & 10 & 20 & 40  & 1 & 5 & 10 & 20 & 40    \\
% %         \midrule
% %         \llama  &\scriptsize{43.5}  &\scriptsize{46.0}  &\scriptsize{47.1} &\scriptsize{46.9} &\scriptsize{46.0}  &\scriptsize{65.7}  &\scriptsize{69.1} &\scriptsize{70.3} &\scriptsize{69.7}&\scriptsize{66.1}  &\scriptsize{33.6}  &\scriptsize{40.2} &\scriptsize{40.2} &\scriptsize{41.0} &\scriptsize{41.9}\\
% %         \llamaone  &\scriptsize{45.1}  &\scriptsize{48.8}  &\scriptsize{48.9} &\scriptsize{48.8} &\scriptsize{47.6}  &\textbf{\scriptsize{66.1}}  &\textbf{\scriptsize{69.4}} &\textbf{\scriptsize{70.4}} &\textbf{\scriptsize{70.9}}&\textbf{\scriptsize{72.1}} &\scriptsize{33.2}  &\scriptsize{39.8} &\scriptsize{41.2} &\scriptsize{42.4} &\scriptsize{42.2}\\
% %         \hdashline
% %         \replug &\scriptsize{12.8}  &\scriptsize{16.9}  &- &- &-  &\scriptsize{23.4}  &\scriptsize{28.7}  &- &- &- &\scriptsize{9.0}  &\scriptsize{13.5}  &- &- &- \\
% %         \replugone &\scriptsize{12.6}  &\scriptsize{17.0}  &\scriptsize{18.9} &- &-  &\scriptsize{23.7}  &\scriptsize{29.1}  &\scriptsize{31.3} &- &- &\scriptsize{8.7}  &\scriptsize{13.8}  &\scriptsize{15.0} &- &- \\
% %         \PAMQA  &\scriptsize{44.1} &\textbf{\scriptsize{51.9}}  &\scriptsize{46.5} &\scriptsize{40.7} &\scriptsize{19.7}  &\scriptsize{61.3}  &\scriptsize{65.9}  &\scriptsize{61.2} &\scriptsize{52.3} &\scriptsize{29.0} &\scriptsize{30.0}  &\scriptsize{37.0} &\scriptsize{35.9} &\scriptsize{34.9} &\scriptsize{15.7} \\
% %         \rowcolor{gray!25}
% %         \kvllamaT  &\scriptsize{44.4} &\scriptsize{51.6}  &\scriptsize{51.7} &\textbf{\scriptsize{51.4}} &\textbf{\scriptsize{49.8}}  &\scriptsize{59.3}  &\scriptsize{69.2}  &\scriptsize{68.9} &\scriptsize{69.7} &\scriptsize{68.5} &\scriptsize{34.0}  &\scriptsize{44.5} &\scriptsize{46.7} &\textbf{\scriptsize{48.3}} &\textbf{\scriptsize{46.7}} \\
% %         \kvllamaoneT  &\textbf{\scriptsize{45.9}} &\scriptsize{51.7}  &\textbf{\scriptsize{51.8}} &\scriptsize{50.8} &\scriptsize{49.0}  &\scriptsize{63.7}  &\scriptsize{68.6}  &\scriptsize{68.3} &\scriptsize{69.3} &\scriptsize{68.7} &\textbf{\scriptsize{35.3}}  &\textbf{\scriptsize{44.7}} &\textbf{\scriptsize{47.6}} &\scriptsize{47.4} &\scriptsize{45.3} \\
% %         \bottomrule
% %     \end{tabularx}
% %     \caption{Accuracy comparison with other position-invariant methods in the RAG pipeline. As top-k increases, baseline models experience a sharp decline in accuracy. In contrast, KV-fusion exhibits a more gradual decrease in accuracy, ranging from 2\% to 5\% between top-20 and top-40 contexts.}
% %     \vspace{-5mm}
% %     \label{tab:exp2}
% % \end{table*}


% % 23.7	29.13	31.33
% % ther methods experience significant performance
% % degradation beyond certain thresholds (likely due to context window limitations), KV-models main-
% % tain consistent accuracy across extended contexts.

% % \begin{table*}[!t]
% %     \renewcommand{\arraystretch}{1.15}
% %     \centering
% %     \small
% %     \begin{tabularx}{\textwidth}{p{2.6cm} XXXXX XXXXX XXXXX c}
% %         \toprule
% %         \textbf{Dataset}    & \multicolumn{5}{c}{\textbf{NQ}}   & \multicolumn{5}{c}{\textbf{TQA}}  & \multicolumn{5}{c}{\textbf{POPQA}} &\multirow{2}{*}{\textbf{\normalsize Gain}}  \\
% %         \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16} 
% %         \textbf{Top-K} & 1 & 5 & 10 & 20 & 40 & 1 & 5 & 10 & 20 & 40  & 1 & 5 & 10 & 20 & 40    &~ \\
% %         % \midrule
% %         % \multicolumn{14}{l}{\llama-2-7B} \\
% %         % \llama  &\scriptsize{43.5}  &\scriptsize{46.0}  &\scriptsize{47.1} &\scriptsize{46.9} &\scriptsize{46.0}  &\scriptsize{65.7}  &\scriptsize{69.1} &\scriptsize{70.3} &\scriptsize{69.7}&\scriptsize{66.1}  &\scriptsize{33.6}  &\scriptsize{40.2} &\scriptsize{40.2} &\scriptsize{41.0} &\scriptsize{41.9}\\
% %         % \llamaone  &\scriptsize{45.1}  &\scriptsize{48.8}  &\scriptsize{48.9} &\scriptsize{48.8} &\scriptsize{47.6}  &\textbf{\scriptsize{66.1}}  &\textbf{\scriptsize{69.4}} &\textbf{\scriptsize{70.4}} &\textbf{\scriptsize{70.9}}&\textbf{\scriptsize{72.1}} &\scriptsize{33.2}  &\scriptsize{39.8} &\scriptsize{41.2} &\scriptsize{42.4} &\scriptsize{42.2}\\
% %         \hdashline
% %         \replug &-  &-  &- &- &-  &-  &-  &- &- &- &-  &-  &- &- &- &- \\
% %         % \replugone &-  &-  &- &- &-  &-  &-  &- &- &- &-  &-  &- &- &- &- \\
% %         \PAMQA  &\scriptsize{44.1} &\textbf{\scriptsize{51.9}}  &\scriptsize{46.5} &\scriptsize{40.7} &\scriptsize{19.7}  &\scriptsize{61.3}  &\scriptsize{65.9}  &\scriptsize{61.2} &\scriptsize{52.3} &\scriptsize{29.0} &\scriptsize{30.0}  &\scriptsize{37.0} &\scriptsize{35.9} &\scriptsize{34.9} &\scriptsize{15.7} &- \\
% %         \rowcolor{gray!25}
% %         \kvllama  &\scriptsize{44.4} &\scriptsize{51.6}  &\scriptsize{51.7} &\textbf{\scriptsize{51.4}} &\textbf{\scriptsize{49.8}}  &\scriptsize{59.3}  &\scriptsize{69.2}  &\scriptsize{68.9} &\scriptsize{69.7} &\scriptsize{68.5} &\scriptsize{34.0}  &\scriptsize{44.5} &\scriptsize{46.7} &\textbf{\scriptsize{48.3}} &\textbf{\scriptsize{46.7}} &+\scriptsize{1.4} \\
% %         \kvllamaone  &\textbf{\scriptsize{45.9}} &\scriptsize{51.7}  &\textbf{\scriptsize{51.8}} &\scriptsize{50.8} &\scriptsize{49.0}  &\scriptsize{63.7}  &\scriptsize{68.6}  &\scriptsize{68.3} &\scriptsize{69.3} &\scriptsize{68.7} &\textbf{\scriptsize{35.3}}  &\textbf{\scriptsize{44.7}} &\textbf{\scriptsize{47.6}} &\scriptsize{47.4} &\scriptsize{45.3} &+\scriptsize{2.5} \\
% %         \bottomrule
% %     \end{tabularx}
% %     \caption{Performance (\%) comparison with other position-invariant RAG pipelines.}
% %     \vspace{-5mm}
% %     \label{tab:exp2}
% % \end{table*}
